Voxel Deformation-Aware Neural Intersection Function

We extend the Locally-Subdivided Neural Intersection Function (LSNIF) to support parameterized deformable and animated geometry. Our approach introduces a rest-space and deformed-space formulation inspired by meshless rendering, allowing ray samples to be mapped back to a canonical space where a single neural network represents geometry consistently across poses without retraining. To maintain accuracy under deformation-aware training, we incorporate scale-invariant distance regression, uncertainty-weighted multi-task learning, and a hybrid positional-grid encoding. The resulting method preserves the compactness and efficiency of LSNIF while enabling robust neural intersection prediction for dynamic geometry.

==> backup.tex <==


%Neural intersection functions offer a compact alternative to traditional geometric acceleration structures. The Locally-Subdivided Neural Intersection Function (LSNIF) achieves high-quality intersection prediction for static objects by learning a voxel-based representation that outputs multiple attributes such as distance, surface normal, albedo, material, and occlusion. However, its applicability to deformable or animated geometry remains limited. In this paper, we extend LSNIF to support deformation of voxelized geometry through a rest-space and deformed-space mapping inspired by meshless rendering techniques. Our formulation enables a single neural model to represent geometry consistently across poses without retraining. In addition, we revise the training objective to improve accuracy and robustness: we replace the standard mean-absolute-error loss with a log-scaled mean-squared-error for distance prediction and introduce an uncertainty-weighted multi-task loss that adaptively balances supervision across predicted attributes. We also combine positional encoding together with grid encoding, which enables the network to better capture spatial variations. The resulting deformation-aware LSNIF maintains the compactness and efficiency of the original method while achieving stable and accurate intersection prediction under deformation.

% Neural intersection functions provide a compact alternative to traditional geometric acceleration structures. The Locally-Subdivided Neural Intersection Function (LSNIF) demonstrates that high-quality object-space intersection queries can be represented by a small neural network trained on voxelized geometry, but it is limited to static objects. In this work, we extend LSNIF to support deformable and animated geometry by introducing a rest-space and deformed-space mapping inspired by meshless rendering. Ray samples are evaluated in deformed space and mapped back to the rest space, allowing a single network to represent geometry consistently across poses without retraining. Supporting deformation requires training on a wide range of poses, which can reduce single-pose accuracy compared to the original LSNIF. To compensate for this increased variability, we introduce three targeted modifications: a log-scaled mean-squared-error loss for stable distance regression, an uncertainty-weighted multi-task objective for adaptive supervision across predicted attributes, and a hybrid positional-grid encoding to better capture spatial variation. Together, these changes preserve the compactness and efficiency of LSNIF while enabling robust and accurate intersection prediction for deformable geometry.


% \section{Introduction}
% Neural representations for geometry and intersection queries have recently shown impressive efficiency and accuracy, which offers a promising alternative to traditional acceleration structures~\cite{10.1145/3528223.3530127}. Specifically, the work of LSNIF demonstrated that object-space intersection queries can be represented by a small neural network trained on voxelized geometry~\cite{10.1145/3728295}. By encoding spatial information via a sparse hash grid, LSNIF learns to predict intersection distance, surface normal, albedo, and occlusion along any query ray. This design enables accurate and compact intersection prediction while eliminating the need for a bottom-level BVH, which achieves significant memory reduction while maintaining high rendering quality. 

% Despite these advantages, current neural intersection methods, including LSNIF, are limited to static geometry.
% However, in practice, scenes often contain deformable or articulated objects whose topology and pose vary over time.
% Handling deformation efficiently remains challenging since neural networks trained on static geometry cannot generalize to new poses or deformed shapes without retraining.
% In classical graphics pipelines, deformation is addressed using skinning, meshless deformation, or volumetric warping, which define a mapping between a rest space and a deformed space.
% In neural representations, however, deformation introduces additional complexity since the geometry is implicit and distributed across network parameters.

% To overcome this limitation, we extend the LSNIF framework to support parameterized deformation of voxelized geometry by adopting the concept of rest space and deformed space from meshless rendering methods~\cite{luton:hal-05095359}. Instead of directly deforming mesh vertices, our approach applies the parameterized deformation field to the voxel domain referenced by LSNIF. Ray samples are traced in the deformed space but mapped back to the rest space before being encoded and processed by the neural network. As a result, a single network trained in rest space can represent geometry consistently across multiple poses, enabling efficient intersection prediction for animated or deformable objects without retraining.


% However, supporting deformation requires modifying the data collection and training procedure to cover a wide range of object poses. This increased variability introduces a trade-off: for single-pose prediction under identical training conditions, the original LSNIF may achieve higher accuracy due to overfitting than a deformation-aware model trained across multiple poses. To compensate for this loss in pose-specific optimality, we introduce three key modifications to improve robustness and learning efficiency.

% First, we revisit the distance prediction formula and its regression objective. The original LSNIF employs a mean-absolute-error (MAE) loss with sigmoid activation, which does not adequately account for the large dynamic range of intersection distances encountered across poses. We replace this with a log-scaled mean-squared-error (log-MSE) loss and pair it with a balanced training dataset that better spans the distance distribution. This change improves numerical stability and reduces sensitivity to large residuals.

% Second, we reformulate training as a multi-task learning problem with uncertainty-based weighting. Each predicted attribute is associated with a learnable uncertainty parameter that dynamically determines its contribution to the total loss. This allows the network to adaptively balance geometry- and appearance-related supervision during optimization, leading to improved convergence and more consistent multi-attribute reconstruction.

% Third, we incorporate positional encoding in conjunction with grid encoding~\cite{tancik2020fourier}. By mapping voxel hit positions into a higher-dimensional sinusoidal representation prior to grid encoding, the network can better capture fine-grained spatial variations and distinguish input features more effectively, which is particularly important under deformation-induced variability.


% In combination, these contributions yield a deformation-aware, uncertainty-adaptive neural intersection function that maintains the compactness and efficiency of LSNIF while achieving robust and accurate intersection prediction for dynamic geometry.




% In summary, this work makes the following contributions:


% \begin{itemize}

% \item \textbf{Deformation-aware LSNIF:}  a rest-deformed-space extension of LSNIF enabling a single model to support parameterized deformation.
% \item \textbf{Log-scaled MSE distance loss:} a scale-invariant and numerically stable objective with balanced sampling that improves distance regression under multi-pose training.

% \item \textbf{Uncertainty-weighted multi-task objective:} learnable task weighting that adaptively balances distance, normal, albedo, material and occlusion predictions.

% \item \textbf{Hybrid positional-grid encoding:} the combination of positional and grid-based encoding to improve spatial fidelity and mitigate accuracy loss from deformation-aware training.


% \end{itemize}


% \begin{itemize}


% a rest-deformed-space extension of LSNIF enabling a single model to support parameterized deformation.


% \item \textbf{Deformation-aware LSNIF:} a rest-deformed-space extension of LSNIF enabling a single model to support parameterized deformation.

% \item \textbf{Log-scaled MSE distance loss:} a numerically stable, scale-invariant distance objective for multi-pose training.

% \item \textbf{Uncertainty-weighted multi-task objective:} adaptive loss weighting for joint prediction of geometry and appearance attributes.

% \item \textbf{Hybrid positional-grid encoding:} combined positional and grid encoding to improve spatial fidelity under deformation.

% \end{itemize}



%In addition to the deformation mechanism, we revisit the training objective of LSNIF. The original implementation employs a single mean-absolute-error (MAE) loss with a sigmoid activation and fixed, equal weights for all predicted attributes. While simple, this loss design does not reflect the distinct characteristics or dynamic range of different outputs. In particular, intersection distances can vary by several orders of magnitude, making them sensitive to scaling and outliers.

%To address this, we replace the distance regression loss with a log-scaled mean-squared-error (log-MSE) and paired it with a balanced training dataset that covers a wider range of distance distribution, which improves numerical stability and reduces the impact of large residuals.

% Furthermore, we reformulate the overall training as a multi-task learning problem with uncertainty-based weighting. we associate each prediction task with a learnable uncertainty parameter that determines its relative contribution to the total loss. This allows the network to dynamically balance geometry- and appearance-related predictions during optimization, which leads to improved convergence and more consistent multi-attribute reconstruction. We additionally incorporate positional encoding, which maps each 3D voxel hit point into a higher-dimensional representation using sinusoidal functions. This encoding is applied prior to grid encoding and enables the network to better capture spatial variations, thereby improving its ability to distinguish input features and enhancing training efficiency. 



% 19th December 2025
% Need to add this idea from Takahiro's suggestion:
% To support deformation, we have to modify the data collection procedure to incorporate a wide variety of poses. Consequently, for single-pose prediction, the classic LSNIF may outperform the deformation-aware model given the same training condition. To compensate for this, we introduce three key modifications: a log-scaled MSE loss, an uncertainty-weighted loss formulation, and a positional grid encoding scheme.
% (Done, in introduction)


% \takahiro{the proposed input encoding described in XX. }
%positional encoding and then queried against a sparse hash grid. 


%  --- (backup)
% Under this mapping, the original straight ray becomes a piecewise curved path in rest space.  We then intersect this curved path with the rest-space geometry to obtain the ground-truth attributes needed for training, including the true hit distance, surface normal, albedo, material, and occlusion. By sampling many deformation parameters and repeating this procedure, we generate a comprehensive dataset that associates deformed-space voxel hits with rest-space ground-truth geometry. 


% \takahiro{it would be better to start describing "obvious" method where we train deformed geometry as they are, which results in training different shapes (also can we do a comparison to this method and show ours is better if we have time and space?). Instead of doing this, we deform the ray so the learned geometry stays the same which we believe (would be great if we can show) produces better quality geometry reconstruction. it is always good to discuss "why" behind the idea. This inverse deformation is common in physics simulation so I'd say I'm inspired by this rather than the HPG paper (which is fine). }
% (Done)


%\takahiro{Computing intersection of curved ray to geometry is computationally expensive, we applied linear approximation in a single voxel where we use straight ray in the rest space. This can be seen as a segmented linear approximation of the original curved ray as shown in Fig. X.}
% (Done)


%\takahiro{the output from this formulation is the same form to LSNIF, but with simply different voxel hit location which are not always on a straight line. }
% (Simplified, done)

% \takahiro{it may be already written but let's clarify we only support parametarized deformation, not free form deformation}
% (Done)

% How the deformation & Hitpoint & Distances are calcualted and rendered


% Action items after review:
% comments: inline the formula (done)
% unocupied voxels : (Done)


%If no hit is detected within a segment, its full length is accumulated and traversal continues. 


% \begin{equation}
% \label{eq:segment_length}
% \ell_i = \lVert \mathbf{x}_i^1 - \mathbf{x}_i^0 \rVert ,
% \qquad
% \delta_i = \lVert \mathbf{x}_i^0 - \mathbf{x}_{i-1}^1 \rVert
% \end{equation}

% \begin{equation}
% \label{eq:segmented_distance}
% D = \sum_{j=0}^{k-1} \left( \delta_j + \ell_j \right) + \delta_k + t_k
% \end{equation}


%\takahiro{these are small enough so we can inline so we can save space.}


% \begin{equation}
% \label{eq:segmented_distance_definitions}
% \begin{aligned}
% \ell_i &= \lVert \mathbf{x}_i^1 - \mathbf{x}_i^0 \rVert,
% &\delta_i &= \lVert \mathbf{x}_i^0 - \mathbf{x}_{i-1}^1 \rVert, \\
% D &= \sum_{j=0}^{k-1} \left( \delta_j + \ell_j \right) + \delta_k + t_k
% \end{aligned}
% \end{equation}


% TODO: we might need a figure here for distnace calculation

% Encoding : PECS + Grid


% We train the network using a multi-task objective with uncertainty-based loss weighting following Kendall et al.~\cite{8578879}. Each predicted attribute is associated with a learnable uncertainty parameter that adaptively balances its contribution during optimization, removing the need for manual loss tuning.

% Let $\mathcal{L}_i$ denote the loss for task $i$ and let $s_i = \log \sigma_i^2$ be a learnable log-variance. For regression tasks, the weighted loss is defined as $\mathcal{L}^{\text{reg}}$ in Eq.~\ref{eq:uncertainty_loss}, while for classification tasks, we use $\mathcal{L}^{\text{cls}}$. The total training objective is the sum of weighted losses over all tasks.

% Compared to LSNIF, we revise the distance prediction formulation. Since deformation yields ray paths composed of multiple segments, the true hit point location can no longer be bounded by a single parameter. We therefore replace the sigmoid output activation with a ReLU and directly regress the distance value. To improve numerical stability over a wide dynamic range, distances are log-transformed and supervised using a mean-squared-error loss in log space. This distance loss is treated as a regression task.

% Surface normals are supervised using a cosine similarity loss between predicted and ground-truth unit vectors. For albedo, we replace the relative $\ell_2$ loss used in LSNIF with an $\ell_1$ loss on sigmoid-activated RGB values. Both normal and albedo losses are treated as regression tasks $\mathcal{L}^{\text{reg}}$ in Eq.~\ref{eq:uncertainty_loss}.


% Material prediction is formulated as a multi-class classification task with cross-entropy loss, while occlusion is modeled as a binary classification task using binary cross-entropy loss. These tasks follow the classification formulation in Eq.~\ref{eq:uncertainty_loss}.


%Compared to LSNIF, which models distance using a sigmoid activation and mean-absolute error (MAE), we revise both the output activation and the loss formulation. Since deformation induces a segmented ray whose total distance is accumulated across multiple segments, the formula to calculate the true hit point location can no longer be bounded by a single parameter. Therefore, We replace the sigmoid activation with a ReLU and regress distance directly.

% To improve numerical stability across a wide dynamic range, we apply a logarithmic transformation to the distance values and use a mean-squared-error loss in log space. This loss is treated as a regression task $\mathcal{L}^{\text{reg}}$ in Eq.~\ref{eq:uncertainty_loss}.



% \begin{equation}
% \label{eq:uncertainty_loss}
% \mathcal{L}_i^{\text{reg}} =
% \frac{1}{2} \exp(-s_i)\,\mathcal{L}_i
% + \frac{1}{2} s_i
% \qquad
% \mathcal{L}_i^{\text{cls}} =
% \exp(-s_i)\,\mathcal{L}_i
% + \frac{1}{2} s_i
% \end{equation}



% \begin{equation}
% \label{eq:uncertainty_regression}
% \mathcal{L}_i^{\text{reg}} =
% \frac{1}{2} \exp(-s_i)\,\mathcal{L}_i
% + \frac{1}{2} s_i
% \end{equation}


% \begin{equation}
% \label{eq:uncertainty_classification}
% \mathcal{L}_i^{\text{cls}} =
% \exp(-s_i)\,\mathcal{L}_i
% + \frac{1}{2} s_i
% \end{equation}

% Gathering training data, balanced sampling and how to apply the reverse transformation (deformed -> rest) ?

% \begin{equation}
% \label{eq:positional_encoding}
% \gamma(\mathbf{x}) =
% \left[
% \mathbf{x},
% \sin\left(2^0 \mathbf{x}\right), \cos\left(2^0 \mathbf{x}\right),
% \ldots,
% \sin\left(2^{F-1} \mathbf{x}\right), \cos\left(2^{F-1} \mathbf{x}\right)
% \right]
% \end{equation}

% \begin{equation}
% \label{eq:positional_encoding}
% \gamma(\mathbf{x}) =
% \left[
% \mathbf{x},
% \{\sin(2^k \mathbf{x}), \cos(2^k \mathbf{x})\}_{k=0}^{F-1}
% \right]
% \end{equation}


% \begin{equation}
% \label{eq:hashgrid_encoding_and_joint_encoding}
% \phi(\mathbf{x}) = \bigoplus_{l=1}^{L} \phi_l(\mathbf{x}),
% \qquad
% \psi(\mathbf{x}) = \phi\bigl(\gamma(\mathbf{x})\bigr)
% \end{equation}



% \begin{subequations}
% \label{eq:encodings}
% \begin{align}
% \gamma(\mathbf{x}) &=
% \left[
% \mathbf{x},
% \{\sin(2^k \mathbf{x}), \cos(2^k \mathbf{x})\}_{k=0}^{F-1}
% \right], \label{eq:positional_encoding} \\
% \phi(\mathbf{x}) &= \bigoplus_{l=1}^{L} \phi_l(\mathbf{x}),
% \qquad
% \psi(\mathbf{x}) = \phi\bigl(\gamma(\mathbf{x})\bigr)
% \label{eq:hashgrid_encoding_and_joint_encoding}
% \end{align}
% \end{subequations}

% \begin{equation}
% \label{eq:hashgrid_encoding}
% \phi(\mathbf{x}) = \bigoplus_{l=1}^{L} \phi_l(\mathbf{x})
% \end{equation}

% \begin{equation}
% \label{eq:joint_encoding}
% \psi(\mathbf{x}) = \phi\bigl(\gamma(\mathbf{x})\bigr)
% \end{equation}


% Loss: Weighted loss 

% Special loss function for distance  (MAE+Sigmoid -> log-scale MSE) + other loss changes


% TODO: maybe we mention how we gather and rebalance the dataset here ?



% \begin{figure}[t]

%     \centering
%     \begin{subfigure}{0.32\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{cat_model2_albedo.png}
%         \caption{Deformed}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.32\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{cat_model3_albedo.png}
%         \caption{Proposed}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.32\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{cat_ref_albedo.png}
%         \caption{Reference}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.32\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{cat_orig.png}
%         \caption{Original}
%     \end{subfigure}


% \caption{Comparison of images illustrating deformation and the improvements our proposed methods bring}
% \label{fig:deformed_final_images}
% \end{figure}


% \begin{figure}[t]
%     \centering
%     \parbox[t]{0.24\linewidth}{\centering
%         \includegraphics[width=\linewidth]{cat_model2_albedo.png}\\
%         \small (a) Deformed}
%     \hfill
%     \parbox[t]{0.24\linewidth}{\centering
%         \includegraphics[width=\linewidth]{cat_model3_albedo.png}\\
%         \small (b) Proposed}
%     \hfill
%     \parbox[t]{0.24\linewidth}{\centering
%         \includegraphics[width=\linewidth]{cat_ref_albedo.png}\\
%         \small (c) Reference}
%     \hfill
%     \parbox[t]{0.24\linewidth}{\centering
%         \includegraphics[width=\linewidth]{cat_orig.png}\\
%         \small (d) Original}

%     \caption{Comparison of images illustrating deformation and the improvements introduced by the proposed method.}
%     \label{fig:deformed_final_images}
% \end{figure}


% \begin{figure}[t]

%     \centering
%     \parbox[t]{0.24\linewidth}{\centering
%         \includegraphics[width=\linewidth]{dragon_model2_material.png}\\
%         \small (a) Deformed}
%     \hfill
%     \parbox[t]{0.24\linewidth}{\centering
%         \includegraphics[width=\linewidth]{dragon_model3_material.png}\\
%         \small (b) Proposed}
%     \hfill
%     \parbox[t]{0.24\linewidth}{\centering
%         \includegraphics[width=\linewidth]{dragon_ref_material.png}\\
%         \small (c) Reference}
%     \hfill
%     \parbox[t]{0.24\linewidth}{\centering
%         \includegraphics[width=\linewidth]{rest_space.png}\\
%         \small (d) Original}

%     \caption{Comparison of images illustrating the prediction of multiple materials under deformation.}
%     \label{fig:deformed_multi_mat_images}
% \end{figure}



% \subsection{Deformation with Global Illumination}

% To integrate the deformation-aware LSNIF into a global illumination rendering pipeline, we follow the same high-level strategy as the original LSNIF while adapting ray traversal to account for deformation. The key challenge is that ray-deformed voxel intersections are calculated in deformed space, whereas intersection prediction is performed by a neural model defined in rest space. For rays that intersect the deformable object, the intersection position is not known a priori. We query the deformation-aware NIF to get the predicted distance $t$ and compute the corresponding hit point $P = O + \mathbf{d}t$. This hit point then serves as the origin for casting secondary rays, including shadow rays, within the global illumination framework.

% (Maybe we should remove this since we only have 4 pages)
% \subsection{Distance Distribution}



% MAE for Distance Bar Plot
% \begin{figure}[h]
%     \centering
%     \begin{tikzpicture}
    
%     \begin{axis}[
%         label style={font=\tiny}, 
%         xbar, 
%         ytick={1,2,3}, 
%         yticklabels={LSNIF, Deformed, Proposed},
%         yticklabel style={align=center, font=\tiny}, 
%         xlabel={Mean Absolute Error (MAE)},
%         x tick label style={font=\tiny}, 
%         xmin=0, xmax=0.16, 
%         bar width=4pt,
%         nodes near coords,
%         every node near coord/.append style={font=\tiny},
%         width=\linewidth,
%         height=2.5cm,
%         enlarge y limits=0.4
%     ]
%     \addplot coordinates {(0.105,1) (0.135,2) (0.039,3)}; 
%     \end{axis}
%     \end{tikzpicture}
%     %\caption{MAE for Distance Comparison}

% %\end{figure}

% % Normal Angular Error Bar Plot 
% %\begin{figure}[h]
% %    \centering

%     \begin{tikzpicture}
%     \begin{axis}[
%         label style={font=\tiny},
%         xbar,
%         ytick={1,2, 3}, 
%         yticklabels={LSNIF, Deformed, Proposed},
%         yticklabel style={align=center, font=\tiny},
%         xlabel={Normal Angular Error (degrees)},
%         x tick label style={font=\tiny},
%         xmin=0, xmax=28.0,
%         bar width=4pt,
%         nodes near coords,
%         every node near coord/.append style={font=\tiny},
%         width=\linewidth,
%         height=2.5cm, 
%         enlarge y limits=0.4,
%     ]
%     \addplot coordinates {(19.1,1) (24.7,2) (11.8,3)};
%     \end{axis}
%     \end{tikzpicture}
    
% \caption{Comparison of prediction performance between LSNIF , the Deformed model and after applying the proposed methods on a single, original pose: Mean Absolute Error (MAE) for distance prediction and Normal Angular Error for normal vector prediction.}

% \label{fig:lsnif_vs_deformed}
% \end{figure}




% Once initialized, traversal proceeds by stepping across voxel boundaries via face-based ray-plane intersection tests. For each hit voxel, we compute the corresponding hit interval and map deformed-space intersections back to rest space for supervision. Traversal terminates upon the first valid hit or when the ray exits the scene bounds.



% Can we extend NifApp ?
% Albedo
% Chessboard texture
% tree-like structure
% Differnet deformation ?

% Comparison
% Training result: Blanced data vs normal data
% Training result: Weighted loss vs equal loss

% Deformation on the mesh for the OGL pipeline ?




%\input{tikz_figs.inc}

% \subsection{Uncertainty-Weighted Multi-Task Loss}


% We adopt an uncertainty-weighted multi-task objective following Kendall et al.~\cite{8578879}, where each prediction task is associated with a learnable uncertainty parameter that dynamically balances its contribution during training.

% Let $\mathcal{L}_i$ denote the loss of task $i$ and let $s_i = \log \sigma_i^2$ be its learnable log-variance. For regression tasks, the weighted loss is defined as
% $\mathcal{L}_i^{\text{reg}} = 0.5\,\exp(-s_i)\,\mathcal{L}_i + 0.5\,s_i$,
% while for classification tasks we use
% $\mathcal{L}_i^{\text{cls}} = \exp(-s_i)\,\mathcal{L}_i + 0.5\,s_i$.
% The total training loss is the sum over all tasks.

% Compared to LSNIF, we revise the distance prediction formulation. Deformation produces ray paths composed of multiple segments, which makes the accumulated distance unbounded. We therefore replace the sigmoid output activation with a ReLU and directly regress the distance. To improve numerical stability across a wide dynamic range, distances are log-transformed and supervised using a mean-squared-error loss in log space, which is treated as a regression task.

% Surface normals are supervised using a cosine similarity loss between predicted and ground-truth unit vectors. Albedo is predicted using sigmoid-activated RGB values and supervised with an $\ell_1$ loss. Both are treated as regression tasks with $\mathcal{L}^{\text{reg}}$.

% Material prediction is formulated as a multi-class classification task with cross-entropy loss, while occlusion is modeled as a binary classification task using binary cross-entropy loss. These tasks follow the classification weighting, $\mathcal{L}^{\text{cls}}$.


% \subsection{Accuracy Comparison without Deformation}

% To isolate the impact of deformation-aware training, we first evaluate our method under a static, single-pose setting and compare it directly against the original LSNIF. In this experiment, both models are evaluated on identical voxelized geometry without applying any deformation, ensuring that differences in performance stem solely from the training strategy rather than pose variation.

% As expected, the original LSNIF achieves slightly higher accuracy in this controlled setting. Because it is trained exclusively on a single pose, the network can overfit to pose-specific geometric and appearance details, resulting in lower distance and normal prediction errors, as shown in Table~\ref{tab:lsnif_vs_deformed}. In contrast, our deformation-aware model is trained on a distribution of poses, even though deformation is not applied at test time. This increased variability acts as a regularizer and limits the network's ability to specialize for a single configuration. More importantly, the accuracy gap observed in the static setting is not only reduced by our proposed modifications, but in several metrics, our method outperforms the original LSNIF, despite being trained for deformation. Figure~\ref{fig:lsnif_vs_deformed_images} illustrates the visual comparison.




% \subsection{Segmented Ray Distance Accumulation}

% Under deformation, a ray that is linear in deformed space becomes piecewise linear when mapped to the rest space. Consequently, intersection distance can no longer be represented by a single ray parameter. We instead define the distance as the accumulated length of ray segments traversed across deformed voxels.

% Voxel traversal produces an ordered sequence of entry-exit point pairs $(\mathbf{x}_i^0, \mathbf{x}_i^1)$ for geometry-occupied voxels in deformed space, where each pair defines a local ray segment with length $\ell_i=\lVert \mathbf{x}_i^1 - \mathbf{x}_i^0 \rVert$ in occupied voxel $i$ and the inter-voxel offset $\delta_i = \lVert \mathbf{x}_i^0 - \mathbf{x}_{i-1}^1 \rVert$ between consecutive segments, as there could be unoccupied voxels in between. Each segment is traced independently against the scene geometry, yielding a local hit distance $t_i \in [0, \ell_i]$ measured from the segment entry point. The total intersection distance $D = \sum_{j=0}^{k-1} \left( \delta_j + \ell_j \right) + \delta_k + t_k$ is then computed by accumulating segment lengths until the first hit occurs, where $k$ denotes the index of the voxel containing the first intersection. During evaluation, hit positions are reconstructed by marching along the same segmented ray and calculating the directions iteratively, ensuring consistency between distance prediction and spatial localization.
